Can Learning to Answer Spatial Questions Improve Novel-View Generation?

Generating novel views from limited observations requires preserving both the appearance and spatial structure of a scene. Although recent approaches exploit fine-grained geometric cues, they do not explicitly model high-level semantic and spatial properties such as object identity, attributes, and inter-object relationships. In this work, we investigate whether 3D language understanding can provide complementary supervision for novel-view generation. We introduce Ask4NV, built on a pretrained unified multimodal model with a Mixture-of-Transformers (MoT) architecture. Our model incorporates camera geometry into both VAE and ViT representations and leverages understanding features during generation through joint self-attention with a modality-aware attention masking strategy. Experiments demonstrate strong image quality and geometric consistency in novel-view generation, alongside competitive 3D language understanding. Further analysis shows that joint training improves cross-view correspondence in VAE representations and similarity in a 3D-aware feature space.

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}


\newcommand{\hlrow}{\rowcolor{black!6}}

\usepackage{colortbl}
\RequirePackage{booktabs}
\usepackage{lipsum}

\usepackage{multirow}

\usepackage{amsmath, amssymb, amsfonts} % For math symbols
\usepackage{graphicx} % Required for \includegraphics (though not used in this text-only example)
\usepackage{bm} % For bold math symbols using \bm
\usepackage{bbm}

% --- Subcaption Configuration ---
% This makes subtables behave like independent tables for numbering
\usepackage{caption}    % Required for \captionof and general caption setup
\usepackage{xcolor}
\usepackage{xspace}
% optional accessibility for cvpr camready pdf readability
\usepackage[accsupp]{axessibility}
% \newcommand{\ours}{ViewPrint\xspace}
\newcommand{\ours}{Ask4NV\xspace}
\usepackage{wrapfig}
% --- Caption Configuration (applies to \captionof{table} and standard table captions) ---
\captionsetup{
  labelfont=bf,  % Makes the label ("Table X") bold
  labelsep=colon % Adds a colon after the label
}
\raggedbottom
% --- End Caption Configuration ---
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}  % 체크마크
\newcommand{\xmark}{\ding{55}} 
% Define some common commands for consistency if you wish
\newcommand{\vect}[1]{\mathbf{#1}} % For vectors (e.g., \vect{x})
\newcommand{\matr}[1]{\mathbf{#1}} % For matrices (e.g., \matr{K})
\newcommand{\set}[1]{\mathcal{#1}} % For sets (e.g., \set{V})
\definecolor{dark_green}{rgb}{0, 0.5, 0}
\definecolor{light_purple}{rgb}{0.6, 0.5, 0.8}

\newcommand{\camready}[1]{{\color{light_purple}#1}}
\newcommand{\davgocc}{\ensuremath{\delta_\text{avg}^\text{occ}}\xspace}
\newcommand{\davgvis}{\ensuremath{\delta_\text{avg}^\text{vis}}\xspace}

\usepackage{xcolor}
\newcommand{\paragrapht}[1]{\noindent\textbf{#1}}

\usepackage{algorithm}
\usepackage{algpseudocode}

\newcommand{\std}{$\mathcal{S}$} 

\usepackage{etoc}      
\usepackage{lineno}   
\usepackage{hyperref}  

\usepackage[most]{tcolorbox}
\definecolor{kblue}{RGB}{0,66,148}

\newcounter{findingcounter}
\newcommand{\finding}[2]{%
  \refstepcounter{findingcounter}%
  \begin{tcolorbox}[
    enhanced jigsaw,
    colback=red!10!white,
    colframe=red!60!black,
    arc=2pt,
    boxsep=3pt,
    left=10pt,
    right=10pt,
    top=3pt,
    bottom=3pt,
    boxrule=0.8pt
  ]
    {\color{black}\bfseries
      Finding~\arabic{findingcounter}.~#1}%
    \enspace #2
  \end{tcolorbox}%
}
